Illuminating Gravitational Waves: A Concordant Picture of Photons from a Neutron Star Merger

Merging neutron stars offer an exquisite laboratory for simultaneously studying strong-field gravity and matter in extreme environments. We establish the physical association of an electromagnetic counterpart EM170817 to gravitational waves (GW170817) detected from merging neutron stars. By synthesizing a panchromatic dataset, we demonstrate that merging neutron stars are a long-sought production site forging heavy elements by r-process nucleosynthesis. The weak gamma-rays seen in EM170817 are dissimilar to classical short gamma-ray bursts with ultra-relativistic jets. Instead, we suggest that breakout of a wide-angle, mildly-relativistic cocoon engulfing the jet elegantly explains the low-luminosity gamma-rays, the high-luminosity ultraviolet-optical-infrared and the delayed radio/X-ray emission. We posit that all merging neutron stars may lead to a wide-angle cocoon breakout; sometimes accompanied by a successful jet and sometimes a choked jet.

==> 2MASS_Tab.tex <==
\begin{tabular}{c c c c c c c c c}
\hline
\multicolumn{1}{c}{2MASS ID} & \multicolumn{1}{c}{RA} & \multicolumn{1}{c}{DEC} & \multicolumn{1}{c}{Jmag} & \multicolumn{1}{c}{eJmag} & \multicolumn{1}{c}{Hmag} & \multicolumn{1}{c}{eHmag} &
\multicolumn{1}{c}{Kmag} & \multicolumn{1}{c}{eKmag}  \\
\hline
13094767-2321594 & 197.455295 & -23.389151 & 14.256 & 0.022 & 13.656 & 0.024 & 13.477 & 0.037 \\
13094842-2323499	& 197.451774	& -23.397219	& 14.435	& 0.032	& 13.870	& 0.043	& 13.746	& 0.043\\
13094767-2321594 & 197.448652	& -23.366512	& 14.669	& 0.035	& 14.102	& 0.048	& 13.728	& 0.043\\
\hline
\end{tabular}

==> CLUmatch.tex <==
\begin{sidewaystable*}
\caption{Census of the Local Universe (CLU) galaxies within the
  localization volume of GW170817 \cite{LVCC21535}.  For each galaxy
  we give the coordinates (J2000), distance, far-ultraviolet (FUV) magnitude from \textit{GALEX}, mid-infrared magnitudes from \textit{WISE}, estimated star-formation rate (SFR) based on the FUV magnitude, estimated stellar mass based on the mid-infrared magnitudes, and probability within the GW170817 localization volume.}
{\small
\begin{tabular}{cccccccccc}
\hline
\hline
Galaxy         & RA	       & DEC	       & $D$   & FUV    & WISE1  & WISE4  & $\log_{10}({\rm SFR})$ (FUV)	         & $\log_{10}(M_\star)$         & Prob.    \\ 
	       & (deg)     & (deg)     & (Mpc) &(AB)    &(Vega)  &(Vega)  &($M_{\odot}$yr$^{-1}$)& ($M_{\odot}$) &  \\ 
\hline

NGC 4970 & 196.8906 & $-$24.0086 & 46.50 & $\ldots$ & \phn9.78 & 8.01 & $\ldots$ & 10.42 & 0.68 \\
NGC 4830 & 194.3663 & $-$19.6913 & 47.90 & 18.88 & \phn9.87 & 8.34 & $-$1.32 & 10.41 & 0.75 \\
NGC 4993 & 197.4487 & $-$23.3839 & 41.66 & 20.13 & \phn9.94 & 7.47 & $-$1.35 & 10.26 & 0.41 \\
NGC 4968 & 196.7749 & $-$23.6770 & 42.24 & 18.93 & \phn9.99 & 2.41 & \phantom{$-$}0.63 & 10.25 & 0.51 \\
IC 4197 & 197.0180 & $-$23.7969 & 43.24 & $\ldots$ & 10.07 & 7.45 & $\ldots$ & 10.24 & 0.48 \\
IC 4180 & 196.7354 & $-$23.9171 & 42.46 & 18.05 & 10.19 & 5.62 & $-$0.58 & 10.17 & 0.60 \\
ESO 508$-$ G 033 & 199.0969 & $-$26.5614 & 45.59 & 17.02 & 10.90 & 3.70 & \phantom{$-$}0.21 & \phn9.95 & 0.83 \\
MCG $-$02$-$33$-$036 & 193.1066 & $-$15.5172 & 53.87 & 19.81 & 11.50 & 7.47 & $-$1.11 & \phn9.86 & 0.88 \\
ESO 508$-$ G 010 & 196.9080 & $-$23.5790 & 43.04 & $\ldots$ & 11.88 & 5.97 & $\ldots$ & \phn9.51 & 0.44 \\
MCG $-$03$-$33$-$023 & 194.2521 & $-$17.3202 & 56.79 & $\ldots$ & 12.93 & 6.37 & $\ldots$ & \phn9.33 & 0.90 \\
ESO 575$-$ G 053 & 196.2705 & $-$22.3839 & 36.37 & 16.46 & 11.98 & 6.47 & $-$0.68 & \phn9.33 & 0.23 \\
2MASX J12525109$-$1529300 & 193.2130 & $-$15.4916 & 52.26 & $\ldots$ & 12.80 & 8.55 & $\ldots$ & \phn9.31 & 0.84 \\
2MASX J12505229$-$1454238 & 192.7180 & $-$14.9066 & 52.96 & 17.92 & 12.89 & 7.10 & $-$0.79 & \phn9.29 & 0.89 \\
2MASX J12573271$-$1942006 & 194.3863 & $-$19.7002 & 52.39 & 20.65 & 12.96 & 9.18 & $-$1.73 & \phn9.25 & 0.87 \\
ESO 576$-$ G 003 & 197.6488 & $-$21.7482 & 42.04 & $\ldots$ & 12.65 & 6.59 & $\ldots$ & \phn9.18 & 0.89 \\
UGCA 331 & 197.6914 & $-$23.8657 & 40.82 & $\ldots$ & 12.61 & 7.33 & $\ldots$ & \phn9.17 & 0.47 \\
IC 3825 & 192.6544 & $-$14.4828 & 51.04 & 18.24 & 13.10 & 7.33 & $-$0.93 & \phn9.17 & 0.87 \\
ESO 575$-$ G 055 & 196.6663 & $-$22.4561 & 44.49 & 17.11 & 13.04 & 7.29 & $-$0.79 & \phn9.07 & 0.32 \\
ESO 508$-$ G 003 & 196.6000 & $-$24.1641 & 40.52 & 16.93 & 12.86 & 6.89 & $-$0.77 & \phn9.06 & 0.73 \\
ESO 508$-$ G 019 & 197.4663 & $-$24.2391 & 41.79 & $\ldots$ & 13.13 & 6.66 & $\ldots$ & \phn8.98 & 0.47 \\
ESO 575$-$ G 029 & 193.9986 & $-$19.2691 & 45.21 & $\ldots$ & 13.36 & 7.96 & $\ldots$ & \phn8.96 & 0.78 \\
2MASX J13073768$-$2356181 & 196.9071 & $-$23.9384 & 49.73 & $\ldots$ & 13.66 & 8.44 & $\ldots$ & \phn8.92 & 0.75 \\
2MFGC 10461 & 197.1774 & $-$23.7756 & 41.39 & $\ldots$ & 13.32 & 8.61 & $\ldots$ & \phn8.90 & 0.40 \\
2MFGC 10484 & 197.4617 & $-$24.2419 & 42.31 & $\ldots$ & 13.46 & $\ldots$ & $\ldots$ & \phn8.86 & 0.48 \\
2MASX J13061939$-$2258491 & 196.5805 & $-$22.9804 & 41.51 & 17.52 & 13.51 & 7.30 & $-$0.96 & \phn8.83 & 0.35 \\
UGCA 327 & 196.9370 & $-$22.8579 & 37.29 & $\ldots$ & 13.33 & 7.02 & $\ldots$ & \phn8.81 & 0.24 \\
GALEXASC J125520.46$-$170546.9 & 193.8364 & $-$17.0966 & 56.69 & 18.39 & 14.58 & 8.31 & $-$1.06 & \phn8.67 & 0.89 \\
WINGS J125412.84$-$153523.6 & 193.5534 & $-$15.5899 & 50.96 & $\ldots$ & 14.43 & 8.33 & $\ldots$ & \phn8.64 & 0.82 \\
ESO 508$-$ G 004 & 196.7177 & $-$22.8405 & 41.37 & 16.59 & 14.05 & 8.54 & $-$0.78 & \phn8.61 & 0.26 \\
ESO 508$-$ G 014 & 197.1342 & $-$23.3469 & 46.61 & 18.44 & 14.32 & 8.83 & $-$1.31 & \phn8.60 & 0.50 \\
%% 6dF J1254495$-$160308 & 193.7063 & $-$16.0523 & 48.02 & $\ldots$ & 14.60 & 8.60 & $\ldots$ & 8.52 & 0.64 \\
%% GALEXASC J125811.97$-$210246.3 & 194.5501 & $-$21.0461 & 43.89 & 17.69 & 14.51 & 8.86 & $-$1.13 & 8.47 & 0.90 \\
%% GALEXASC J130525.30$-$233008.8 & 196.3546 & $-$23.5025 & 45.90 & 17.44 & 14.73 & 7.16 & $-$0.83 & 8.43 & 0.76 \\
%% GALEXASC J125259.36$-$152150.9 & 193.2474 & $-$15.3639 & 49.87 & 18.44 & 14.96 & 8.63 & $-$1.23 & 8.41 & 0.78 \\
%% GALEXASC J125301.39$-$151007.7 & 193.2552 & $-$15.1693 & 53.40 & 20.94 & 15.25 & 8.93 & $-$1.67 & 8.35 & 0.90 \\
%% PGC45429 & 196.7822 & $-$24.1104 & 41.50 & $\ldots$ & 14.82 & 9.12 & $\ldots$ & 8.30 & 0.65 \\
%% 6dF J1305235$-$233121 & 196.3478 & $-$23.5224 & 41.71 & 17.31 & 14.90 & 8.41 & $-$1.02 & 8.28 & 0.68 \\
%% UGCA 325 & 196.7796 & $-$24.1119 & 42.70 & $\ldots$ & 15.05 & $\ldots$ & $\ldots$ & 8.24 & 0.67 \\
%% GALEXASC J130415.26$-$225251.3 & 196.0633 & $-$22.8814 & 41.23 & 18.41 & 15.05 & 8.72 & $-$1.40 & 8.20 & 0.57 \\
%% 6dF J1309177$-$242256 & 197.3241 & $-$24.3821 & 40.36 & $\ldots$ & 15.23 & 7.34 & $\ldots$ & 8.12 & 0.49 \\
%% UGCA 328 & 197.3298 & $-$24.3866 & 41.03 & $\ldots$ & 15.27 & 8.31 & $\ldots$ & 8.11 & 0.50 \\
%% GALEXASC J125157.02$-$160617.8 & 192.9872 & $-$16.1047 & 50.30 & 21.04 & 15.85 & 8.20 & $-$1.49 & 8.06 & 0.76 \\
%% ESO 508$-$ G 035 & 199.4497 & $-$26.9025 & 37.77 & 17.95 & 15.33 & 9.19 & $-$1.37 & 8.02 & 0.85 \\
%% PGC45611 & 197.3286 & $-$24.3846 & 39.81 & 15.87 & 15.55 & 8.29 & $-$0.54 & 7.98 & 0.49 \\
% {ABELL 1664\_11:[PSE2006] 2506} & 196.8922 & $-$23.8153 & 42.80 & 21.49 & 15.83 & 9.09 & $-$1.96 & 7.93 & 0.50 \\
% GALEXASC J131426.62$-$271242.6 & 198.6106 & $-$27.2120 & 29.32 & 18.39 & 15.28 & 8.77 & $-$1.69 & 7.82 & 0.89 \\
% {ABELL 1631:[CZ2003]B0295[024]} & 192.8695 & $-$15.8723 & 53.56 & $\ldots$ & 16.70 & 8.46 & $\ldots$ & 7.77 & 0.87 \\
% WINGS J125701.38$-$172325.2 & 194.2558 & $-$17.3903 & 26.13 & $\ldots$ & 16.83 & 9.31 & $\ldots$ & 7.10 & 0.27 \\
% HIPASS J1255$-$15 & 193.8983 & $-$15.0175 & 27.32 & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & 0.00 & 0.83 \\
\hline
%\input{tables/table1.txt}

\label{tab:clumatch}
\end{tabular}
}
\end{sidewaystable*}

\begin{sidewaystable*}
\contcaption{Census of the Local Universe (CLU) galaxies within the localization volume of GW170817 \cite{LVCC21535}, continued.}
{\small
\begin{tabular}{cccccccccc}
\hline
\hline
Galaxy         & RA	       & DEC	       & $D$   & FUV    & WISE1  & WISE4  & $\log_{10}({\rm SFR})$ (FUV)	         & $\log_{10}(M_\star)$         & Prob.    \\ 
	       & (deg)     & (deg)     & (Mpc) &(AB)    &(Vega)  &(Vega)  &($M_{\odot}$yr$^{-1}$)& ($M_{\odot}$) &  \\ 
\hline

% NGC 4970 & 196.8906 & $-$24.0086 & 46.50 & $\ldots$ & 9.78 & 8.01 & $\ldots$ & 10.42 & 0.68 \\
% NGC 4830 & 194.3663 & $-$19.6913 & 47.90 & 18.88 & 9.87 & 8.34 & $-$1.32 & 10.41 & 0.75 \\
% NGC 4993 & 197.4487 & $-$23.3839 & 41.66 & 20.13 & 9.94 & 7.47 & $-$1.35 & 10.26 & 0.41 \\
% NGC 4968 & 196.7749 & $-$23.6770 & 42.24 & 18.93 & 9.99 & 2.41 & \phantom{$-$}0.63 & 10.25 & 0.51 \\
% IC 4197 & 197.0180 & $-$23.7969 & 43.24 & $\ldots$ & 10.07 & 7.45 & $\ldots$ & 10.24 & 0.48 \\
% IC 4180 & 196.7354 & $-$23.9171 & 42.46 & 18.05 & 10.19 & 5.62 & $-$0.58 & 10.17 & 0.60 \\
% ESO 508$-$ G 033 & 199.0969 & $-$26.5614 & 45.59 & 17.02 & 10.90 & 3.70 & \phantom{$-$}0.21 & 9.95 & 0.83 \\
% MCG $-$02$-$33$-$036 & 193.1066 & $-$15.5172 & 53.87 & 19.81 & 11.50 & 7.47 & $-$1.11 & 9.86 & 0.88 \\
% ESO 508$-$ G 010 & 196.9080 & $-$23.5790 & 43.04 & $\ldots$ & 11.88 & 5.97 & $\ldots$ & 9.51 & 0.44 \\
% MCG $-$03$-$33$-$023 & 194.2521 & $-$17.3202 & 56.79 & $\ldots$ & 12.93 & 6.37 & $\ldots$ & 9.33 & 0.90 \\
% ESO 575$-$ G 053 & 196.2705 & $-$22.3839 & 36.37 & 16.46 & 11.98 & 6.47 & $-$0.68 & 9.33 & 0.23 \\
% 2MASX J12525109$-$1529300 & 193.2130 & $-$15.4916 & 52.26 & $\ldots$ & 12.80 & 8.55 & $\ldots$ & 9.31 & 0.84 \\
% 2MASX J12505229$-$1454238 & 192.7180 & $-$14.9066 & 52.96 & 17.92 & 12.89 & 7.10 & $-$0.79 & 9.29 & 0.89 \\
% 2MASX J12573271$-$1942006 & 194.3863 & $-$19.7002 & 52.39 & 20.65 & 12.96 & 9.18 & $-$1.73 & 9.25 & 0.87 \\
% ESO 576$-$ G 003 & 197.6488 & $-$21.7482 & 42.04 & $\ldots$ & 12.65 & 6.59 & $\ldots$ & 9.18 & 0.89 \\
% UGCA 331 & 197.6914 & $-$23.8657 & 40.82 & $\ldots$ & 12.61 & 7.33 & $\ldots$ & 9.17 & 0.47 \\
% IC 3825 & 192.6544 & $-$14.4828 & 51.04 & 18.24 & 13.10 & 7.33 & $-$0.93 & 9.17 & 0.87 \\
% ESO 575$-$ G 055 & 196.6663 & $-$22.4561 & 44.49 & 17.11 & 13.04 & 7.29 & $-$0.79 & 9.07 & 0.32 \\
% ESO 508$-$ G 003 & 196.6000 & $-$24.1641 & 40.52 & 16.93 & 12.86 & 6.89 & $-$0.77 & 9.06 & 0.73 \\
% ESO 508$-$ G 019 & 197.4663 & $-$24.2391 & 41.79 & $\ldots$ & 13.13 & 6.66 & $\ldots$ & 8.98 & 0.47 \\
% ESO 575$-$ G 029 & 193.9986 & $-$19.2691 & 45.21 & $\ldots$ & 13.36 & 7.96 & $\ldots$ & 8.96 & 0.78 \\
% 2MASX J13073768$-$2356181 & 196.9071 & $-$23.9384 & 49.73 & $\ldots$ & 13.66 & 8.44 & $\ldots$ & 8.92 & 0.75 \\
% 2MFGC 10461 & 197.1774 & $-$23.7756 & 41.39 & $\ldots$ & 13.32 & 8.61 & $\ldots$ & 8.90 & 0.40 \\
% 2MFGC 10484 & 197.4617 & $-$24.2419 & 42.31 & $\ldots$ & 13.46 & $\ldots$ & $\ldots$ & 8.86 & 0.48 \\
% 2MASX J13061939$-$2258491 & 196.5805 & $-$22.9804 & 41.51 & 17.52 & 13.51 & 7.30 & $-$0.96 & 8.83 & 0.35 \\
% UGCA 327 & 196.9370 & $-$22.8579 & 37.29 & $\ldots$ & 13.33 & 7.02 & $\ldots$ & 8.81 & 0.24 \\
% GALEXASC J125520.46$-$170546.9 & 193.8364 & $-$17.0966 & 56.69 & 18.39 & 14.58 & 8.31 & $-$1.06 & 8.67 & 0.89 \\
% WINGS J125412.84$-$153523.6 & 193.5534 & $-$15.5899 & 50.96 & $\ldots$ & 14.43 & 8.33 & $\ldots$ & 8.64 & 0.82 \\
% ESO 508$-$ G 004 & 196.7177 & $-$22.8405 & 41.37 & 16.59 & 14.05 & 8.54 & $-$0.78 & 8.61 & 0.26 \\
% ESO 508$-$ G 014 & 197.1342 & $-$23.3469 & 46.61 & 18.44 & 14.32 & 8.83 & $-$1.31 & 8.60 & 0.50 \\
6dF J1254495$-$160308 & 193.7063 & $-$16.0523 & 48.02 & $\ldots$ & 14.60 & 8.60 & $\ldots$ & \phn8.52 & 0.64 \\
GALEXASC J125811.97$-$210246.3 & 194.5501 & $-$21.0461 & 43.89 & 17.69 & 14.51 & 8.86 & $-$1.13 & \phn8.47 & 0.90 \\
GALEXASC J130525.30$-$233008.8 & 196.3546 & $-$23.5025 & 45.90 & 17.44 & 14.73 & 7.16 & $-$0.83 & \phn8.43 & 0.76 \\
GALEXASC J125259.36$-$152150.9 & 193.2474 & $-$15.3639 & 49.87 & 18.44 & 14.96 & 8.63 & $-$1.23 & \phn8.41 & 0.78 \\
GALEXASC J125301.39$-$151007.7 & 193.2552 & $-$15.1693 & 53.40 & 20.94 & 15.25 & 8.93 & $-$1.67 & \phn8.35 & 0.90 \\
PGC45429 & 196.7822 & $-$24.1104 & 41.50 & $\ldots$ & 14.82 & 9.12 & $\ldots$ & \phn8.30 & 0.65 \\
6dF J1305235$-$233121 & 196.3478 & $-$23.5224 & 41.71 & 17.31 & 14.90 & 8.41 & $-$1.02 & \phn8.28 & 0.68 \\
UGCA 325 & 196.7796 & $-$24.1119 & 42.70 & $\ldots$ & 15.05 & $\ldots$ & $\ldots$ & \phn8.24 & 0.67 \\
GALEXASC J130415.26$-$225251.3 & 196.0633 & $-$22.8814 & 41.23 & 18.41 & 15.05 & 8.72 & $-$1.40 & \phn8.20 & 0.57 \\
6dF J1309177$-$242256 & 197.3241 & $-$24.3821 & 40.36 & $\ldots$ & 15.23 & 7.34 & $\ldots$ & \phn8.12 & 0.49 \\
UGCA 328 & 197.3298 & $-$24.3866 & 41.03 & $\ldots$ & 15.27 & 8.31 & $\ldots$ & \phn8.11 & 0.50 \\
GALEXASC J125157.02$-$160617.8 & 192.9872 & $-$16.1047 & 50.30 & 21.04 & 15.85 & 8.20 & $-$1.49 & \phn8.06 & 0.76 \\
ESO 508$-$ G 035 & 199.4497 & $-$26.9025 & 37.77 & 17.95 & 15.33 & 9.19 & $-$1.37 & \phn8.02 & 0.85 \\
PGC45611 & 197.3286 & $-$24.3846 & 39.81 & 15.87 & 15.55 & 8.29 & $-$0.54 & \phn7.98 & 0.49 \\
{ABELL 1664\_11:[PSE2006] 2506} & 196.8922 & $-$23.8153 & 42.80 & 21.49 & 15.83 & 9.09 & $-$1.96 & \phn7.93 & 0.50 \\
GALEXASC J131426.62$-$271242.6 & 198.6106 & $-$27.2120 & 29.32 & 18.39 & 15.28 & 8.77 & $-$1.69 & \phn7.82 & 0.89 \\
{ABELL 1631:[CZ2003]B0295[024]} & 192.8695 & $-$15.8723 & 53.56 & $\ldots$ & 16.70 & 8.46 & $\ldots$ & \phn7.77 & 0.87 \\
WINGS J125701.38$-$172325.2 & 194.2558 & $-$17.3903 & 26.13 & $\ldots$ & 16.83 & 9.31 & $\ldots$ & \phn7.10 & 0.27 \\
HIPASS J1255$-$15 & 193.8983 & $-$15.0175 & 27.32 & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & \phn0.00 & 0.83 \\

\hline
%\input{tables/table1.txt}
%\label{tab:clumatch}
\end{tabular}
}
\end{sidewaystable*}



